Tools for Analyzing Parallel I/O

Parallel application I/O performance often does not meet user expectations. Additionally, slight access pattern modifications may lead to significant changes in performance due to complex interactions between hardware and software. These challenges call for sophisticated tools to capture, analyze, understand, and tune application I/O. In this paper, we highlight advances in monitoring tools to help address this problem. We also describe best practices, identify issues in measurement and analysis, and provide practical approaches to translate parallel I/O analysis into actionable outcomes for users, facility operators, and researchers.

==> uniform_analysis.tex <==
\subsection{Unifying Trace Analysis}
With storage systems increasing in size and the use case of a single system being so diverse, especially in the scientific community, it is paramount we understand the behavior of such systems. Understanding system behavior helps light the path for future storage system development, and allows for the purveyors of these systems to ensure performance is adequate to allow for work to continue unimpeded. While most systems in industry are well understood, shared parallel file systems in the high performance computing (HPC) community are not as well understood. This is due to their large size and many users, which typically submit disperate workloads. For this reason, great effort is put into understanding them, usually with a per system effort using ad-hoc analysis of their system behavior, otherwise known as ad-hoc trace analysis. This work is usually done in an ad-hoc manner because of the nature of the logs produced by these large scale machines - they are machine specific, and despite having similar attributes, do not share a single format for their trace behavior. This extends past HPC storage, and applies more broadly to HPC in general, and additionally, individual application traces.

Because of this difference in log/trace format, system analysis is usually done per system. This can produce useful results on the behavior of a particular system, but sheds no light on how it compares to other similar systems, HPC or otherwise \cite{adams_usage_2012,adams_analysis_2012, wang_file_nodate, noauthor_analysis_nodate}. Additionally, programmer effort is wasted analyzing each system, when the generated analytics are the same or similar for each system. However, due to the difference in traces and techniques, these are not typically comparable, leading to most systems being analyzed in a vacuum, never compared to one another. 

As computing centers grown in size, and the HPC community approaches exascale \cite{bergman2008exascale}, it has become increasingly important to understand how these systems are operating, and how they are being used. We must standardize our approaches to system analysis, both to allow comparison between like systems, and to avoid the programming overhead of repeatedly creating the same analytics code again and again. By doing so, we hope to create a standardized method of analyzing storage systems, as well as other system traces, and light the path forward to exascale and help computing centers deal with massive growth \cite{benson_understanding_2009, peters_eos_2015, bergman2008exascale, peters_exabyte_2011}. Additionally, by creating a general purpose method of trace analysis, we can provide optimizations and features that would be too costly to develop for ad-hoc analysis. This also has use outside of the storage and HPC community, with massive amounts of traces being generated from user applications and other sources.

\iffalse
Note to authors, this is pulled from my masters report, please let me know if this is an issue.

In understanding the performance of parallel I/O it is common to study the behavior of large scale storage systems on their own \cite{adams_usage_2012,adams_analysis_2012, wang_file_nodate, noauthor_analysis_nodate}. Performing this analysis assists in developing new HPC storage systems and expand existing ones.
\fi

==> uniform_tool.tex <==
\subsection{Tools for Unifying Trace Formats}

\jk{Existing approaches like TAU usw.}
\jk{We sounds like the gang of authors, maybe they?}

Work is being done at the University of California, Santa Cruz (UCSC) to produce a tool that provides field per record access to traces with the ability to convert them to another trace schema format through a simple programming language that has been developed for this purpose. By giving the ability to translate traces directly to other formats, there is the expectation that analysis will not be done ad-hoc for different storage systems. This would enable the creation of a standard set of tools for analyzing the behavior of parallel file systems, which we hope to provide in future work.

While the database community has allowed programmable data presentation for some time \cite{smith_guide_nodate}, through views and computed columns, these techniques have not worked their way into trace analysis, despite many system traces being stored in database formats, such as \texttt{Parquet}, a Spark SQL queryable columnar format \cite{parquetwebpage, armbrust_spark_2015}. We believe that presenting data in a uniform format, similar to a trace, is essential, but does not require the overhead of a database, as most analysis is done in place, usually in a time series format. We are aware of the availability of time series databases, but due to indexes only existing on a single time value, they do not serve our purpose \cite{bonnet_towards_2001}. Additionally, because the size and due to the fact these traces grow continually, we do not want to constantly ingest this data into a database. For that reason, we have explored NoDB systems \cite{alagiannis_nodb:_2012, alagiannis_nodb_2012, karpathiotakis_adaptive_2014, tahara_sinew:_2014}, which allow for data to be queried in its raw format, without defined schema.

The trace unification tool being developed borrows techniques from NoDB systems as well as from the database community at large. Because of the sequential nature and read only analysis properties of trace analysis, we must only provide a way to provide low latency translation from one format to another. We believe this is crucial to presenting a uniform format for trace analysis, instead creating a mechanism for schema translation (which we consider to be similar to computed columns in a full database engine that gives the tools necessary to present uniform versions of each trace without storing their information in a database or requiring views to be created before analysis. The goal of this tool is to create an information addressing system that allows for schemas to be translated as data is fetched from its base format with low overhead. Such a system can be used to unify traces based on the information they share, and allow for the information to be analyzed directly, either from a storage system trace analysis tool that we plan to create, or from an API that we plan to add in future work.

This system ingests minimal information about each file to allow for field-per-record addressing, which we believe will be the best interface for analysis tools to access trace data in. We use our mechanism of trace addressing to create field and record primitives, which we use as the basis for our schema translation language. By allowing for records and fields to be used as primitives, we provide a simple mechanism for traces to be unified. We have designed a simple translation language based on s-expressions that allows for simple translation to occur, with more functionality coming in future work. Currently, our method for doing so is focused at the trace analysis community, though in future work we plan to provide additional functionality to allow for more complex translations to occur.

